Geometry-aware training of factorized layers in tensor Tucker format

Reducing parameter redundancies in neural network architectures is crucial for achieving feasible computational and memory requirements during training and inference phases. Given its easy implementation and flexibility, one promising approach is layer factorization, which reshapes weight tensors into a matrix format and parameterizes them as the product of two small rank matrices. However, this approach typically requires an initial full-model warm-up phase, prior knowledge of a feasible rank, and it is sensitive to parameter initialization. In this work, we introduce a novel approach to train the factors of a Tucker decomposition of the weight tensors. Our training proposal proves to be optimal in locally approximating the original unfactorized dynamics independently of the initialization. Furthermore, the rank of each mode is dynamically updated during training. We provide a theoretical analysis of the algorithm, showing convergence, approximation and local descent guarantees. The method's performance is further illustrated through a variety of experiments, showing remarkable training compression rates and comparable or even better performance than the full baseline and alternative layer factorization strategies.

==> tables/table_cifar10.tex <==
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.8} % Default value: 1
\begin{table}[h]
    \centering
    \caption{VGG16 and Alexnet on Cifar10 dataset. }
\begin{NiceTabular}{ll|ccc}
\toprule   
{}& & test acc.[\%] & \multicolumn{2}{c}{compression rate} \\ 
 \cmidrule{4-5}
 & method &  (to baseline) & eval[\%] & train[\%] \\ 
\midrule
\multirow{22}{*}{$\;$\rotatebox[origin=c]{90}{VGG16\!\!\!\!\!\!}}
&{Baseline}&$82.88 \pm 0.23\%$ & \multicolumn{2}{c}{$0.0\%$} \\[0.8em] 
	        
& TDLRT $ \tau = 0.02$ &    $82.86 \pm 1.6$  &$93.57 \pm 0.12$&$50.25 \pm 1.16$ \\      
& TDLRT $ \tau = 0.03$ &    ${83.97} \pm 0.57$  &$95.34 \pm 0.20$&$69.92 \pm 2.09$ \\ 
&  TDLRT $ \tau = 0.04$ &    $82.25 \pm 0.49$  &$96.71 \pm 0.22$&$84.25 \pm 2.12$ \\ 
&  TDLRT $ \tau = 0.05$ &   $81.04 \pm 0.49$  &$97.40 \pm 0.10$&${90.33} \pm 0.85$ \\ 
& TDLRT $ \tau = 0.06$ &    $80.70 \pm 0.47$  &$97.62 \pm 0.04$&$92.38 \pm 0.46$ \\ 
&  TDLRT $ \tau = 0.1$ & $77.80 \pm 0.90$&$98.01 \pm 0.08$&$95.51 \pm 0.53$ \\ 
&  TDLRT $ \tau = 0.15$ &  $74.52 \pm 1.04$ &$ 98.23 \pm 0.02$& $96.67 \pm 0.12$  \\[.8em]

    & CP-factorized $\kappa=0.95$ & $72.28 \pm 1.89$& \multicolumn{2}{c}{$93.64$} \\ 
    & CP-factorized $\kappa=0.9$  & $75.89 \pm 1.57$& \multicolumn{2}{c}{$88.73$} \\ 
    & CP-factorized $\kappa=0.8$  & $77.13 \pm 2.71$& \multicolumn{2}{c}{$78.86$} \\ 
    & CP-factorized $\kappa=0.6$  & $77.62 \pm 4.36$& \multicolumn{2}{c}{$59.12$} \\[.8em]
    & Tucker-factorized $\kappa=0.95$ & $57.92 \pm 1.91 $& \multicolumn{2}{c}{$93.39$} \\
    & Tucker-factorized $\kappa=0.9$ & $59.10 \pm 3.79 $& \multicolumn{2}{c}{$89.03$} \\
    & Tucker-factorized $\kappa=0.8$ & $75.95 \pm 4.65 $& \multicolumn{2}{c}{$75.26$} \\
    & Tucker-factorized $\kappa=0.6$ & $77.19 \pm 1.05 $& \multicolumn{2}{c}{$61.34$} \\
    & Tucker-factorized $\kappa=0.4$ & $78.42 \pm 0.96 $& \multicolumn{2}{c}{$52.32$} \\[.8em]
   & Matrix-factorized $\kappa=0.95$ & $68.23 \pm 1.47$& \multicolumn{2}{c}{$92.90$} \\
   & Matrix-factorized $\kappa=0.9$& $73.41 \pm 2.12$& \multicolumn{2}{c}{$87.20$} \\
   & Matrix-factorized $\kappa=0.8$ & $78.32 \pm 4.03$& \multicolumn{2}{c}{$75.78$} \\
   & Matrix-factorized $\kappa=0.6$ & $81.25 \pm 0.19$& \multicolumn{2}{c}{$52.26$} \\[.8em]
   &  DLRT & $82.58 \pm 0.20$&$83.22$&$74.3$ \\
\midrule
\multirow{21}{*}{$\;$\rotatebox[origin=c]{90}{Alexnet\!\!\!\!\!\!}}
&{Baseline}&$79.63 \pm 0.30$ & \multicolumn{2}{c}{$0.0$}\\[0.8em]
	        
        %  &DLRT $\tau =0.04$ &  $76.92 \pm 0.35\%$  &$74.3 \pm 0.25\%$&$-85.18 \pm 3.44\%$ \\ 
	       %  \\
        % &DLRT $\tau =0.05$ &  $77.56 \pm 0.32\%$  &$79.3 \pm 0.31\%$&$-17.6 \pm 3.83\%$ \\ 
	       %  \\
        &TDLRT $\tau =0.06$ &   $76.56 \pm 0.45$  &$83.12\pm 0.80$&$29.82\pm 8.72$ \\ 
	    
	&TDLRT $\tau =0.1$  &$74.92 \pm0.40$&$86.98 \pm 0.08$&$72.42 \pm 0.98$ 
		    \\
      &TDLRT $\tau =0.15$  &$71.34 \pm0.31$&$91.78 \pm 0.09$&$78.60 \pm 0.73$ 
		    \\[.8em]
    & CP-factorized $\kappa=0.95$ & $48.93 \pm 3.23$& \multicolumn{2}{c}{$84.91$} \\ 
    & CP-factorized $\kappa=0.9$ & $56.94 \pm 3.10$& \multicolumn{2}{c}{$80.42$} \\ 
    & CP-factorized $\kappa=0.8$ & $70.31 \pm 0.58$& \multicolumn{2}{c}{$71.46$} \\ 
    & CP-factorized $\kappa=0.7$ & $72.41 \pm 0.44$& \multicolumn{2}{c}{$53.56$} \\[0.8em]

    & Tucker-factorized $\kappa=0.95$ & $50.90 \pm 3.91$& \multicolumn{2}{c}{$84.66$} \\
    & Tucker-factorized $\kappa=0.9$ & $55.14 \pm 1.19$& \multicolumn{2}{c}{$80.53$} \\
    & Tucker-factorized $\kappa=0.8$ & $64.47 \pm 1.92$& \multicolumn{2}{c}{$69.74$} \\
    & Tucker-factorized $\kappa=0.6$ & $71.54 \pm 1.10$& \multicolumn{2}{c}{$54.95$} \\[0.8em]

   & Matrix-factorized $\kappa=0.95$ & $58.87 \pm 0.85$& \multicolumn{2}{c}{$84.07$} \\
   & Matrix-factorized $\kappa=0.9$ & $62.48 \pm 1.45$& \multicolumn{2}{c}{$78.84$} \\
   & Matrix-factorized $\kappa=0.8$ & $71.24 \pm 0.91$& \multicolumn{2}{c}{$68.20$} \\[0.8em]

    &  DLRT & $67.74 \pm 0.19$&$71.57$&$55.5$ \\
 \bottomrule
  % \label{tab:cifar10}
\end{NiceTabular}
% \caption{VGG16 and Alexnet on Cifar10 dataset.}
    \label{tab:cifar10}
\end{table}

==> tables/table_cifar10_short_new.tex <==
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{0.8} % Default value: 1+
% \resizebox{0.48\textwidth}{!}
\resizebox{1\textwidth}{!}
 {
\begin{NiceTabular}{ll| cc cc cc}
\toprule   
& &\multicolumn{2}{c}{VGG16}  & \multicolumn{2}{c}{Alexnet} & \multicolumn{2}{c}{ResNet18}\\
 \cmidrule{3-8}
& & test acc. [\%] & c.r. [\%] &  test acc. [\%] &c.r. [\%] & test acc. [\%] & c.r. [\%] \\ 
 %\cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} 
 \midrule
& Baseline &$89.43$ &$0.0$  &$85.46$ &$0.0$  &$94.33$ & $0.0$ \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{Factorization}} &\textbf{TDLRT} (ours)  &  $\textbf{89.59}$ &$\textbf{95.34}$  &   $\textbf{82.39}$  & $\textbf{83.12}$ & $\textbf{92.72}$ & $78.73$  \\ 
& Matrix DLRT \cite{Schothoefer_2022}& $89.13 $ & $83.22$ & $73.57$ & $71.57$ &  $80.98$ &$56.85$ \\ 
% \midrule
&  Tucker-factorized \cite{kim2016compression} & $83.74 $ & $61.34$ & $ 70.30$ & $69.74 $ & $ 91.11$ & $74.19$\\
&  Matrix-factorized \cite{wang2021pufferfish} & $79.96 $ & $87.20$ & $77.07 $ & { $68.20 $} &$92.07$  &{$77.49$}\\
&  CP-factorized \cite{lebedev2015speedingup} & $83.68$ & {$78.85$} & $ 76.14$& {$ 71.46$} & $ 91.87$& {$ 69.95$} \\ 
 &Tucker RGD \cite{vandereycken2013low} & 81.48 & 84.26 & 73.88 & 74.01 & 92.76 & 74.18 \\
  &      TT-factorized \cite{novikov2015tensorizing} & 87.96 & 84.06 & 78.13 & 88.14 & 87.13 & 81.24 \\
 \midrule
%{Baseline (SNIP)}&$93.18$ &\multicolumn{2}{c}{$0.0$}  &$85.88$ &\multicolumn{2}{c}{$0$} &n.a. &\multicolumn{2}{c}{n.a.} \\
\multirow{3}{*}{\rotatebox[origin=c]{90}{Pruning}} & {SNIP} \cite{lee2019snip} & $89.58$ &{$56.23$}  &$-$ &{$-$} & $89.50$ & $78.50$ \\
& IMP \cite{frankle2018lottery} & $87.21$ &{$58.54$}  &$-$ &{$-$} & $90.50$ & $\textbf{82.50}$ \\
& GraSP \cite{wang2020picking} & $88.50$ &{$77.30$}  &$-$ &{$-$} & $89.40$ & $77.90$ \\
 \bottomrule
\end{NiceTabular}
}
% $89.14$ &{$95.0$}%

% \begin{NiceTabular}{|l|ccc|ccc|ccc|}
% \toprule   
% &\multicolumn{3}{c}{VGG16}  & \multicolumn{3}{c}{Alexnet} & \multicolumn{3}{c}{ResNet18}\\
%  \cmidrule{2-4}  \cmidrule{5-7}\cmidrule{8-10}
% &  & \multicolumn{2}{c}{compression rate [\%]} &  &\multicolumn{2}{c}{compression rate [\%]}&&\multicolumn{2}{c}{compression rate [\%]} \\ 
%  \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} 
%  method & test acc. [\%]  & eval & train & test acc. [\%]  & eval & train & test acc. [\%]  & eval & train\\ 
%  \midrule
% {Baseline}&$89.43$ &\multicolumn{2}{c}{$0.0$}  &$85.46$ &\multicolumn{2}{c}{$0$} &$94.33$ &\multicolumn{2}{c}{$0$} \\
% \midrule
% TDLRT  &  $\textbf{89.59}$ &$\textbf{95.34}$& $69.92$  &   $\textbf{82.39}$  & $\textbf{83.12}$ & $29.82$ & $\textbf{92.72}$ & $78.73$ & $50.80$ \\ 
% Matrix DLRT & $89.13 $ & $83.22$ & $74.30$ & $73.57$ & $71.57$ & $55.51$ & $80.98$ &$56.85$ &$13.71$ \\ 
% \midrule

%  Tucker-factorized & $83.74 $ & \multicolumn{2}{c}{$61.34$} & $ 70.3$ & \multicolumn{2}{c}{$69.74 $}& $ 91.11$ & \multicolumn{2}{c}{$74.19$}\\
%  Matrix-factorized & $79.96 $ & \multicolumn{2}{c}{$87.20$} & $77.07 $ & \multicolumn{2}{c}{ $68.20 $} &$92.07$  &\multicolumn{2}{c}{$77.49$}\\
%  CP-factorized & $83.68$ & \multicolumn{2}{c}{$78.85$} & $ 76.14$& \multicolumn{2}{c}{$ 71.46$} & $ 91.87$& \multicolumn{2}{c}{$ 69.95$} \\ 
%  \midrule
% %{Baseline (SNIP)}&$93.18$ &\multicolumn{2}{c}{$0.0$}  &$85.88$ &\multicolumn{2}{c}{$0$} &n.a. &\multicolumn{2}{c}{n.a.} \\
% {SNIP}&$89.14$ &\multicolumn{2}{c}{$95.0$}  &$84.59$ &\multicolumn{2}{c}{$90$} &n.a. &\multicolumn{2}{c}{n.a.} \\
%  \bottomrule
% \end{NiceTabular}
% }
\label{tab_cifar}


==> tables/table_fmnist.tex <==
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{0.8} % Default value: 1

% \begin{table}[h!]
%     \centering
%     \caption{Lenet5 on Fashion-Mnist dataset.}
% \begin{NiceTabular}{|ll|ccc|}
% \toprule   
% \multicolumn{5}{c}{Lenet5 FASHION MNIST}\\
% \midrule
% {}& & test acc.[\%] & \multicolumn{2}{c}{convolutions compression rate} \\ 
%  \cmidrule{4-5}
%  & method &  (to baseline) & eval[\%] & train[\%] \\ 
% \midrule
% % \multirow{15}{*}{$\;$\rotatebox[origin=c]{90}{Lenet5\!\!\!\!\!\!}}
% &{Baseline}&$90.86\pm0.10$ &$0.0$&$0.0$\\ 
	        
%          % &DLRT $\tau =0.04$ &  $90.17\pm0.24\%$  &$76.74\pm3.77\%$&$-225.52\pm62.65\%$ \\ 
% 	        % \\
%          % &DLRT $\tau =0.05$ &  $90.33\pm0.17\%$  &$84.16\pm0.85\%$&$-102.78\pm13.46\%$ \\ 
% 	        % \\
%         &TDLRT $\tau =0.1$ &  $87.42\pm0.73$  &$94.42\pm0.17$&$64.10\pm3.13$ \\ 
	        
%         &TDLRT $\tau =0.15$ &   $88.89\pm0.19$  &$96.92\pm0.11$&$92.58\pm0.71$ \\ 
	        
% 	&TDLRT $\tau =0.2$  &$88.86\pm0.11$&$97.00 \pm 0.05$&$93.14\pm0.05$ \\ 
		   
%      &TDLRT $\tau =0.3$ &  $88.71\pm0.04$&$97.10\pm0.02$&$94.20\pm 0.01$ 
%          \\
% \midrule
%     & CP-factorized & $89.36 \pm 0.16$&$96.81$&$ 96.81$ \\ 
%    &  Tucker-factorized & $89.14 \pm 0.21$&$96.80$&$96.80$ \\
%     &  Matrix-factorized & $87.47 \pm 0.15$&$91.88$&$91.88$ \\

%  \bottomrule
% %  \label{tab:fmnist}
% %  \caption{Lenet5 on Fashion-Mnist.}
% \end{NiceTabular}
% % \caption{Lenet5 on Fashion-Mnist dataset.}
%     \label{tab:fmnist}
% \end{table}



%%%%% not stds


\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.8} % Default value: 1

\begin{table}[h!]
    \centering
    \caption{Lenet5 on Fashion-Mnist dataset.}
\begin{NiceTabular}{ll|ccc}
\toprule   
{}& & test acc.[\%] & \multicolumn{2}{c}{convolutions compression rate} \\ 
 \cmidrule{4-5}
 & method &  (to baseline) & eval[\%] & train[\%] \\ 
\midrule
% \multirow{15}{*}{$\;$\rotatebox[origin=c]{90}{Lenet5\!\!\!\!\!\!}}
&{Baseline}&$90.86$ &$0.0$&$0.0$\\ 
	        
         % &DLRT $\tau =0.04$ &  $90.17\pm0.24\%$  &$76.74\pm3.77\%$&$-225.52\pm62.65\%$ \\ 
	        % \\
         % &DLRT $\tau =0.05$ &  $90.33\pm0.17\%$  &$84.16\pm0.85\%$&$-102.78\pm13.46\%$ \\ 
	        % \\
        &TDLRT $\tau =0.1$ &  $87.42$  &$94.427$&$64.10$ \\ 
	        
        &TDLRT $\tau =0.15$ &   $88.89$  &$96.921$&$92.58$ \\ 
	        
	&TDLRT $\tau =0.2$  &$88.86$&$97.00$&$93.14$ \\ 
		   
     &TDLRT $\tau =0.3$ &  $88.71$&$97.10$&$94.20$ 
         \\
\midrule
    & CP-factorized & $89.36$&$96.81$&$ 96.81$ \\ 
   &  Tucker-factorized & $89.14$&$96.80$&$96.80$ \\
    &  Matrix-factorized & $87.47$&$91.88$&$91.88$ \\

 \bottomrule
%  \label{tab:fmnist}
%  \caption{Lenet5 on Fashion-Mnist.}
\end{NiceTabular}
% \caption{Lenet5 on Fashion-Mnist dataset.}
    \label{tab:fmnist}
\end{table}

==> tables/table_mnist.tex <==
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{0.8} % Default value: 1

% \begin{table}[h]
% \centering
% \caption{Lenet5 on MNIST dataset}
% \begin{NiceTabular}{|ll|ccc|}
% \toprule   
% \multicolumn{5}{c}{Lenet5 MNIST}\\
% \midrule
% {}& & test acc.[\%] & \multicolumn{2}{c}{convolutions compression rate} \\ 
%  \cmidrule{4-5}
%  & method &  (to baseline) & eval[\%] & train[\%] \\ 
% \midrule
% % \multirow{10}{*}{$\;$\rotatebox[origin=c]{90}{MNIST\!\!\!\!\!\!}}
% &{Baseline}&$98.14 \pm 0.02$ &$0.0$&$0.0$  \\ 
	        
%         % & DLRT $ \tau = 0.1$ &    $\textbf{98.14} \pm0.03\%$  &$89.34 \pm 0.35\%$&$-17.34 \pm 5.0\%$\\ 
% 	       %  \\
%         &  TDLRT $ \tau = 0.15$ &    $97.54\pm0.27$  &$93.76\pm0.52$&$54.02 \pm 7.60$ \\ 
	        
%         &  TDLRT $ \tau = 0.2$ &   $97.80\pm0.08 $&$96.13 \pm 0.26$&$84.64 \pm 3.09$ \\ 
	        
% 		 &  TDLRT $ \tau = 0.3$ & $97.83 \pm 0.11$&$96.52 \pm 0.16$&$89.83 \pm 1.56$ \\  
% \midrule
%    & CP-factorized & $97.56 \pm 0.16$&$99.35$&$ 99.35$ \\ 
%    & Tucker-factorized & $97.97 \pm 0.12$&$96.52$&$93.51$ \\ 
%       & Matrix-factorized & $97.53 \pm 0.19$&$93.40$&$93.40$ \\
		
% \bottomrule
% %  \label{tab:mnist}
% %  \caption{Lenet5 on MNIST dataset.}
% \end{NiceTabular}
% % \caption{Lenet5 on MNIST dataset}
%     \label{tab:mnist}
% \end{table}



\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.8} % Default value: 1

\begin{table}[h]
\centering
\caption{Lenet5 on MNIST dataset}
\begin{NiceTabular}{ll|ccc}
\toprule   
{}& & test acc.[\%] & \multicolumn{2}{c}{convolutions compression rate} \\ 
 \cmidrule{4-5}
 & method &  (to baseline) & eval[\%] & train[\%] \\ 
\midrule
% \multirow{10}{*}{$\;$\rotatebox[origin=c]{90}{MNIST\!\!\!\!\!\!}}
&{Baseline}&$98.14$ &$0.0$&$0.0$  \\ 
	        
        % & DLRT $ \tau = 0.1$ &    $\textbf{98.14} \pm0.03\%$  &$89.34 \pm 0.35\%$&$-17.34 \pm 5.0\%$\\ 
	       %  \\
        &  TDLRT $ \tau = 0.15$ &    $97.54$  &$93.76$&$54.02$ \\ 
	        
        &  TDLRT $ \tau = 0.2$ &   $97.80 $&$96.13$&$84.64 $ \\ 
	        
		 &  TDLRT $ \tau = 0.3$ & $97.83 $&$96.52 6$&$89.83 $ \\  
\midrule
   & CP-factorized & $97.56$&$99.35$&$ 99.35$ \\ 
   & Tucker-factorized & $97.97$&$96.52$&$93.51$ \\ 
      & Matrix-factorized & $97.53$&$93.40$&$93.40$ \\
		
\bottomrule
%  \label{tab:mnist}
%  \caption{Lenet5 on MNIST dataset.}
\end{NiceTabular}
% \caption{Lenet5 on MNIST dataset}
    \label{tab:mnist}
\end{table}
